Interaction-aware Conformal Prediction for Crowd Navigation

During crowd navigation, robot motion plan needs to consider human motion uncertainty, and the human motion uncertainty is dependent on the robot motion plan. We introduce Interaction-aware Conformal Prediction (ICP) to alternate uncertainty-aware robot motion planning and decision-dependent human motion uncertainty quantification. ICP is composed of a trajectory predictor to predict human trajectories, a model predictive controller to plan robot motion with confidence interval radii added for probabilistic safety, a human simulator to collect human trajectory calibration dataset conditioned on the planned robot motion, and a conformal prediction module to quantify trajectory prediction error on the decision-dependent calibration dataset. Crowd navigation simulation experiments show that ICP strikes a good balance of performance among navigation efficiency, social awareness, and uncertainty quantification compared to previous works. ICP generalizes well to navigation tasks under various crowd densities. The fast runtime and efficient memory usage make ICP practical for real-world applications. Code is available at https://github.com/tedhuang96/icp.

==> secs/Supplementary_Material.tex <==
\begin{table*}[hbt!]
% \caption{Performance of ICP with and without Regularization. \textcolor{red}{How to measure the change of conformal prediction radius? Difference of initial and final radius? The ratio of conformal interval radius change with respect to the initial one?}}\label{table-quantitative}
\caption{Performance of ICP with and without Regularization. \textcolor{red}{To be moved to supplementary material if needed. Will not be discussed.}}\label{table-quantitative}
\begin{center}
\begin{tabular}{c|c|ccccccc}
    \hline
    Method & Reg & SR$\uparrow$ & ITR$\downarrow$ & SD$\uparrow$ & PL$\downarrow$ & NT$\downarrow$ & CR \\
    \hline
    ICP$_1$ & & 0.97 & 0.16$\pm$0.13 & 1.31$\pm$0.17 & 12.57$\pm$0.57 & 11.07$\pm$1.19 & 0.93$\pm$0.05 \\
    ICP$_1$ & $\checkmark$ & 0.98 & 0.15$\pm$0.12 & 1.32$\pm$0.16 & 12.59$\pm$0.67 & 11.12$\pm$1.25 & 0.93$\pm$0.05 \\
    \hline
\end{tabular}
\end{center}
\end{table*}
